Integrating Planning and Predictive Control Using the Path Feasibility Governor

The motion planning problem of generating dynamically feasible, collision-free trajectories in non-convex environments is a fundamental challenge for autonomous systems. Decomposing the problem into path planning and path tracking improves tractability, but integrating these components in a theoretically sound and computationally efficient manner is challenging. We propose the Path Feasibility Governor (PathFG), a framework for integrating path planners with nonlinear Model Predictive Control (MPC). The PathFG manipulates the reference passed to the MPC controller, guiding it along a path while ensuring constraint satisfaction, stability, and recursive feasibility. The PathFG is modular, compatible with replanning, and improves computational efficiency and reliability by reducing the need for long prediction horizons. We prove safety and asymptotic stability with a significantly expanded region of attraction, and validate its real-time performance through simulated case studies of unicycle and quadrotor navigation in cluttered environments. \c{opyright}2026 IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works.

==> preamble.tex <==
\makeatletter

\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{physics}
\usepackage{braket}
\usepackage{xparse}
\usepackage[scr=boondox]{mathalpha}
\usepackage{graphicx}
\usepackage{caption3}
\renewcommand\caption@documentclass{standard} % warning suppression
\usepackage[size=footnotesize, list=off]{caption}
\usepackage[size=footnotesize]{subcaption}
\usepackage{tikz}
\usepackage[export]{adjustbox}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage[noadjust]{cite}
\usepackage[dvipsnames]{xcolor}
\usepackage[unit-mode=match]{siunitx}
\usepackage[hidelinks]{hyperref}
\usepackage{enumitem}
\usepackage[tracking]{microtype}
\usepackage{cleveref}
\usepackage{ninecolors}


\newcommand\thespace{\fontdimen2\font plus \fontdimen3\font minus \fontdimen4\font}
\newcommand\thmsep{0.25\baselineskip plus 0.1\baselineskip minus 0.1\baselineskip}

\let\@upn=\relax % use italic numbers in theorems
\declaretheoremstyle[
    spaceabove    = \thmsep,
    spacebelow    = \thmsep,
    headfont      = \itshape,
    notefont      = \itshape,
    notebraces    = {\textnormal(}{\textnormal)},
    headpunct     = {\textnormal:},
    postheadspace = \thespace,
]{theorem_style}
\declaretheorem[style=theorem_style]{theorem}
\declaretheorem[style=theorem_style]{lemma}
\declaretheorem[style=theorem_style]{remark}
\declaretheorem[style=theorem_style]{proposition}
\declaretheorem[style=theorem_style, numbered=no]{claim}
\declaretheorem[style=theorem_style]{corollary}
\declaretheorem[style=theorem_style, name=Assumption]{assume}
\declaretheorem[style=theorem_style, name=Remark]{rmk}

\newlist{assumelist}{enumerate}{1}
\setlist[assumelist]{label={\Alph{*})}, ref=\arabic{assume}\Alph{*}, beginpenalty=10000}
\pretocmd\assumelist{\leavevmode}{}{}

\let\proof=\undefined
\declaretheoremstyle[
    spaceabove    = \thmsep,
    spacebelow    = \thmsep,
    headfont      = \itshape,
    notefont      = \itshape,
    numbered      = no,
    qed           = $\blacksquare$,
    postheadspace = \thespace
]{proof_style}
\declaretheorem[style=proof_style]{proof}

\DeclareMathOperator*\argmin{argmin}
\DeclareMathOperator\Int{int}

\NewDocumentCommand\inv{s}{
    \scriptscriptstyle
    \IfBooleanTF{#1}%
        {\raisebox{0.3ex}{$\scriptscriptstyle-\mspace{-2mu}1$}}%
        {-\mspace{-2mu}1}%
    \mspace{-2mu}\egroup
}
\pretocmd\inv{\bgroup}{}{}

\NewDocumentCommand\?{}{\!\!}
\RenewDocumentCommand\_{O{3} m}{_{\mspace{-#1mu}#2}}
\NewDocumentCommand{\wh}{m}{\widehat{#1}\vphantom{#1}}

\ExplSyntaxOn
\tl_set:Nn \g_transpose_check_tokens_tl {
    {\egroup 3} {\bigr 3} {\right 3} {) 3} {] 3} {\} 3} {\Xi 3}
    {A -3} {P -1} {, -3} {R -1}
}
\NewDocumentCommand \T { s O{3} } {
    \IfBooleanTF { #1 } {
        \mspace { -#2mu } \top \! \c_group_end_token
    } {
        \mspace { -#2mu } \top \c_group_end_token \! \peek_after:Nw \__transpose_aux:
    }
}
\cs_new:Nn \__transpose_aux: {
    \tl_map_inline:Nn \g_transpose_check_tokens_tl {
        \exp_args:Ne \token_if_eq_meaning:NNT { \tl_head:n { ##1 } } \l_peek_token {
            \mspace { \use_none:n ##1 mu } \scan_stop: \tl_map_break:
        }
    }
}
\pretocmd \T { \c_group_begin_token } { } { }
\ExplSyntaxOff

\savebox\@tempboxa{$ $}
\savebox\@tempboxa{\the\textfont1\char"18\char\skewchar\textfont1}
\newlength\xiskew
\setlength\xiskew{\wd\@tempboxa}
\savebox\@tempboxa{\the\textfont1\char"18\kern0pt\char\skewchar\textfont1}
\addtolength\xiskew{-\wd\@tempboxa}
\NewCommandCopy\oldtilde{\tilde}
\RenewDocumentCommand\tilde{m}{%
    \csname tl_if_eq:nnTF\endcsname{\xi}{#1}{%
        \rlap{\kern\xiskew\raisebox{-0.1ex}{$\tilde{\phantom{\xi}}$}}\xi
    }{\oldtilde{#1}}%
}

\NewDocumentCommand\termset{}{\mathcal{T}}
\NewDocumentCommand\phdot{}{\nonscript\+\cdot\nonscript\+}
\NewDocumentCommand\+{}{\mspace{2mu}}
\NewDocumentCommand\p{}{\mathscr{p}}
\NewDocumentCommand\xcentering{}{%
    \centering
    \leftskip=0pt plus 1fil minus \maxdimen
    \rightskip=0pt plus 1fil minus \maxdimen
}
\NewDocumentCommand\noDisplaySkip{s s}{%
    \IfBooleanTF{#1}{\vadjust}{\vadjust pre}% I don't know if IfBooleanTF is expandable or not (I could've put the \vadjust in front)
    {\vspace{\abovedisplayshortskip-\belowdisplayskip}}%
    \IfBooleanT{#2}{\vadjust pre{\vspace{\abovedisplayshortskip-\belowdisplayskip}}}%
}
\NewDocumentCommand\defas{}{\triangleq}
\let\oldepsilon=\epsilon
\RenewDocumentCommand\epsilon{}{\varepsilon}
\RenewDocumentCommand\limsup{}{\varlimsup}
\AtBeginDocument{\RenewDocumentCommand\ref{}{\ifmmode\errmessage{\string\ref\space is prohibited in math mode}\fi\labelcref}}
\RenewDocumentCommand\qty{s}{\quantity}
\NewDocumentCommand\subtext{}{\mathrm}
\NewDocumentCommand\mat{}{\mqty}
\NewDocumentCommand\conjtext{m}{\quad\text{#1}\quad} % replaces \qqtext
\NewDocumentCommand\plus{}{{\scriptscriptstyle+}\@ifnextchar,{\!}{\@ifnextchar-{\!}{}}}
\NewDocumentCommand\dash{}{\unskip\penalty\exhyphenpenalty\textemdash}
\DeclareMathOperator\closure{cl}
\RenewDocumentCommand\emptyset{}{\varnothing}
\let\oldcomplement=\complement
\RenewDocumentCommand\complement{}{{\mspace{1mu}\scalebox{1}[0.85]{$\scriptstyle\oldcomplement$}}}
\colorlet{textcolor}{black}
\definecolor{goodnotesblue}{HTML}{007AFF}

\newcommand\crefrangeconjunction{--}
\medmuskip=4mu plus 1mu minus 3.5mu
\thickmuskip=5mu plus 1.5mu minus 2mu
\setlist[itemize,1]{label=$\vcenter{\hbox{\scriptsize\textbullet}\vspace{-1.5pt}}$}
\setlist[itemize,2]{label=$\vcenter{\hbox{\textbf{--}}\vspace{-1.5pt}}$}
\hyphenation{work-flow Path-FG lem-ma Crazy-flie}
% \begin{luacode}
%     function kernSubscripts(buffer)
%         s = string.gsub(buffer, "\\mathcal O_j", "\\mathcal O_{\\mspace{-2mu}j}")
%         s = string.gsub(s, "_%{\\mathcal O_%{\\mspace%{%-2mu%}j%}%}%(", "_{\\mathcal O_{\\mspace{-2mu}j}\\!}(")
%         s = string.gsub(s, "x_s", "x_{\\mspace{-2mu} s}")
%         s = string.gsub(s, "PathFG%+MPC", "PathFG+\\allowbreak MPC")
%         s = string.gsub(s, "%$N%$%-", "$N\\!$-")
%         return s
%     end
%     luatexbase.add_to_callback("process_input_buffer", kernSubscripts, "kernSubscripts")
% \end{luacode}
\setlength\textfloatsep{1.55\baselineskip plus 3\baselineskip minus 0.4\baselineskip}
\interdisplaylinepenalty=200
\predisplaypenalty=1000
\binoppenalty=700
\relpenalty=500
\hyphenpenalty=100
\doublehyphendemerits=200
\finalhyphendemerits=0
\vbadness=300
\hbadness=300
\RenewDocumentCommand\@IEEEsectpunct{}{\textnormal:\ \,}
\setlength\lineskip{1pt}
\setlength\lineskiplimit{1pt}
\setlength\normallineskip{1pt}
\setlength\normallineskiplimit{1pt}
\RenewDocumentCommand\subsection{}{\@startsection{subsection}{2}{0pt}{1.5ex plus 2ex minus 0.3ex}{0.5ex plus 0.5ex minus 0.2ex}{\normalfont\normalsize\itshape}}
\RenewDocumentCommand\section{}{\@startsection{section}{1}{0pt}{2.5ex plus 2ex minus 0.5ex}{0.7ex plus 0.5ex minus 0.2ex}{\normalfont\normalsize\centering\scshape}}
\setlength\abovedisplayskip{1ex plus 4bp minus 2bp}
\setlength\belowdisplayskip{\abovedisplayskip}
\setlength\belowdisplayshortskip{\abovedisplayskip}
\setlength\abovedisplayshortskip{0pt plus 4bp}
\setlength\jot{1.5pt}

\renewcommand\alglinenumber[1]{\footnotesize#1\ }
\algblockdefx{Substeps}{EndSubsteps}[1]{#1:}{}
\algblockdefx{While}{EndWhile}[1]{while #1 do}{}
\algtext*{EndSubsteps}
\algtext*{EndWhile}
\algrenewcommand\algorithmicfor{\textnormal{for}}
\algrenewcommand\algorithmicdo{\textnormal{do}}

\RenewDocumentCommand\implies{}{%
    \mathchoice
        {\;\Longrightarrow\;}%
        {\,\Rightarrow\,}%
        {\Rightarrow}%
        {\Rightarrow}%
}
\let\oldforall=\forall
\let\oldexists=\exists
\RenewDocumentCommand\forall{}{\oldforall\+}
\RenewDocumentCommand\exists{}{\oldexists\+}
\RenewDocumentCommand\colon{}{%
    \mspace{1mu}\mathpunct{}\nonscript\mspace{-\thinmuskip}%
    \mathord{:}%
    \mspace{6mu plus 1mu}%
}
